CPO: Change Robust Panorama to Point Cloud Localization

We present CPO, a fast and robust algorithm that localizes a 2D panorama with respect to a 3D point cloud of a scene possibly containing changes. To robustly handle scene changes, our approach deviates from conventional feature point matching, and focuses on the spatial context provided from panorama images. Specifically, we propose efficient color histogram generation and subsequent robust localization using score maps. By utilizing the unique equivariance of spherical projections, we propose very fast color histogram generation for a large number of camera poses without explicitly rendering images for all candidate poses. We accumulate the regional consistency of the panorama and point cloud as 2D/3D score maps, and use them to weigh the input color values to further increase robustness. The weighted color distribution quickly finds good initial poses and achieves stable convergence for gradient-based optimization. CPO is lightweight and achieves effective localization in all tested scenarios, showing stable performance despite scene changes, repetitive structures, or featureless regions, which are typical challenges for visual localization with perspective cameras. Code is available at \url{https://github.com/82magnolia/panoramic-localization/}.

==> 3_method.tex <==
\section{Method}
\label{sec:method}



CPO is a panorama to point cloud localization algorithm that explicitly models scene changes using color distribution consistency.
Given a point cloud $P=\{X, C\}$ and a query panorama image $I_{q} \in \mathbb{R}^{H\times W \times 3}$, where $X, C \in \mathbb{R}^{N\times 3}$ are the point cloud coordinates and color values, CPO aims to find the optimal rotation $R^* \in SO(3)$ and translation $t^* \in \mathbb{R}^{3}$ at which the image $I_{q}$ is taken.
As shown in Figure~\ref{fig:overview}, CPO operates by first creating a 2D/3D score map, followed by pose selection using histogram intersections and pose refinement.
The 2D score map $M_{2D} \in \mathbb{R}^{H \times W \times 1}$ and 3D score map $M_{3D} \in \mathbb{R}^{N \times 1}$ measure the color consistency between the panorama and point cloud.
The maps are used to guide the subsequent optimization process of CPO.


\paragraph{Candidate Pose Selection}
To select promising candidate poses for further optimization, we propose a fast and effective pose selection algorithm.
The pose selection algorithm first generates a pool of camera poses from which the candidate poses are chosen.
We construct the space of possible poses in a three-step procedure, where $N_t$ translations are filtered to $N_f$ translations for which $N_r$ rotations are tested.
The initial $N_t$ translations are centroids of the octree or uniform grid partitions of the point cloud, depending on the scene type.
We mainly use octrees for indoor scenes to efficiently partition empty spaces as in Rodenberg \etal~\cite{octree}, and uniform grids for outdoor scenes.
Such a distinction is made because indoor scenes contain numerous clutters that make grid-based partitioning inefficient whereas uniform grids suffice for outdoor scenes lacking clutters.

$N_t$ translations are further filtered to $N_f$ translations by comparing the color histogram intersection of the synthetic view at each location with the panorama image.
Using the filtered translations we evaluate the color histogram intersections of $N_f \times N_r$ poses, where $N_r$ rotations assigned to each translation are uniformly sampled from $SO(3)$.
We bypass the need to render $N_f \times N_r$ synthetic views by using the fast histogram generation procedure explained in Section~\ref{sec:fast}.
The final $K$ poses having the largest histogram intersections with the query panorama image are selected for further pose refinement.
Here, we utilize the 2D score map $M_{2D}$ and place smaller weights on image regions that are likely to contain scene change.
We provide further details about this procedure in Section~\ref{sec:score}.

\paragraph{Pose Refinement}
We individually refine the selected $K$ poses by optimizing a weighted variant of sampling loss~\cite{piccolo}, which quantifies the color difference between 2D and 3D.
To elaborate, let $\Pi(\cdot)$ be the projection function that maps a point cloud to coordinates in the 2D panorama image $I_\text{q}$.
Further, let $\Gamma(\cdot;I_\text{q})$ indicate the sampling function that maps 2D coordinates to pixel values sampled from $I_\text{q}$.
The weighted sampling loss enforces each 3D point's color to be similar with its 2D projection's sampled color, while placing lesser weight on points that are likely to contain change.
Given the 3D score map $M_\text{3D}$, this is expressed as follows,
\begin{equation}
    \label{eq:samp_loss}
    L_\mathrm{sampling}(R, t) = \|M_\text{3D} \odot [\Gamma(\Pi(RX+t);I_\text{q}) - C]\|_2,
\end{equation}
where $\odot$ is the Hadamard product and $RX + t$ is the transformed point cloud under the candidate camera pose $R, t$.
To obtain the refined poses, we minimize the weighted sampling loss values for the $K$ candidate poses using gradient descent~\cite{adam}.
At termination, the refined pose with the smallest sampling loss value is chosen.
In this section we further explain the two key components of CPO: fast histogram generation (Section~\ref{sec:fast}) and score map generation (Section~\ref{sec:score}).

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/figure2.png}
    \caption{Description of fast color histogram generation.}
    \label{fig:hist}
\end{figure}

\subsection{Fast Histogram Generation}
\label{sec:fast}
Efficient generation of color histograms is one of the major building blocks for CPO.
Our histogram generation is formulated using image patches and the 2D geometry of their centroid locations.
As shown in Figure~\ref{fig:hist}, we generate local color histograms over mutually exclusive image patches instead of generating a single global histogram for the entire image.
Such a design choice allows for obtaining color features without sacrificing the rich spatial context in panorama images.

We first explain the generation mechanism under the general case of creating the histogram for a novel view $I_\text{n}$ with known relative pose to the original view $I_\text{o}$.
As shown in Figure~\ref{fig:hist}, let $\mathcal{S}_\text{o}=\{S^o_i\}$ denote the image patches of $I_\text{o}$ and $\mathcal{C}_\text{o}=\{c_i^o\}$ the 2D image coordinates of the patch centroids.
$\mathcal{S}_\text{n}, \mathcal{C}_\text{n}$ is similarly defined for the novel view $I_\text{n}$.
We compute the color histogram for each patch in $\mathcal{S}_\text{o}$, and cache the histograms to synthesize histograms for patches $\mathcal{S}_\text{n}$ in the novel view.
For each novel view patch, we obtain the color histogram by warping the patch centroids to the original view $I_\text{o}$ and using nearest neighbor interpolation.
To elaborate, we first map the patch centroid location $c_i^n$ of $S_i^n \in \mathcal{S}_\text{n}$ to the original image coordinate frame, namely
\begin{equation}
\label{eq:warp}
    p_\text{i} = \Pi(R_\text{rel}\Pi^{-1}(c_i^n) + t_\text{rel}),
\end{equation}
where $R_\text{rel}, t_\text{rel}$ is the relative pose and $\Pi^{-1}(\cdot): \mathbb{R}^{2}\rightarrow \mathbb{R}^{3}$ is the inverse projection function that maps a 2D coordinate to its 3D world coordinate.
The color histogram for $S_i^n$ is assigned as the color histogram of the patch centroid in $I_\text{o}$ that is closest to $p_\text{i}$, namely $c_* = \argmin_{c \in \mathcal{C_\text{o}}} \|c - p_\text{i}\|_2$.

We now illustrate the efficient generation of $N_f \times N_r$ histograms used for candidate pose selection.
Recall that we use color histograms of synthetic views at various locations within the scene to select poses for refinement.
For $N_f$ candidate translations, we evaluate color histograms of $N_r$ rotations.
Since rendering all $N_f \times N_r$ views is expensive, we only render $N_f$ synthetic views and cache the color histogram to generate $N_r$ color histograms for each translation.
Given a synthetic view at a fixed translation, the color histogram for an arbitrary rotation could be generated by warping the patch centroids and performing nearest neighbor interpolation.
Note that in this case computing the warped coordinates in Equation~\ref{eq:warp} does not require the knowledge of depth as only rotation is involved.
The fast generation of color histograms at synthetic views allow for efficient candidate pose selection, which is quantitatively verified in Section~\ref{exp:abl}.

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}

   \caption{Description of 2D score map generation.}
   \label{fig:score2d}
\end{figure}

\subsection{Score Map Generation}
\label{sec:score}
We generate 2D, 3D score maps for change-robust localization based on the color histogram information of the query image and synthetic views from the point cloud.
The color histograms follow the patch-based formulation from Section~\ref{sec:fast} and are generated for virtual camera poses with varying translation and rotation.

\paragraph{Notations} Before we explain the score map generation in detail, we introduce several notations.
Let $\mathcal{Y}$ be the set of synthetic views used for score map creation.
Further, as shown in Figure~\ref{fig:score2d}, let $h_i(\cdot): \mathbb{R}^{H \times W \times 3} \rightarrow \mathbb{R}^B$ be the histogram function that maps a panorama image $I$ to its $\text{i}^\text{th}$ patch color histogram, where B is the number of histogram bins.
Finally, we define the histogram intersection $\Lambda(\cdot, \cdot): \mathbb{R}^B \times \mathbb{R}^B \rightarrow \mathbb{R}$ as the common area between two histograms.

\paragraph{2D Score Map} 
The 2D score map $M_\text{2D} \in \mathbb{R}^{H \times W}$ assigns higher scores to regions in the query image $I_\text{q}$ that are consistent with the point cloud color.
As shown in Figure~\ref{fig:score2d}, we split $M_\text{2D}$ into patches and assign a single score to each patch.
We define the 2D score as the maximum intersection between the patches of the query image $I_\text{q}$ and synthetic views in $\mathcal{Y}$.
Formally, denoting $\mathcal{M}=\{M_i\}$ as the scores for patches in $M_\text{2D}$, the score for the $\text{i}^\text{th}$ patch is
\begin{equation}
\label{eq:2d}
    M_i = \max_{Y \in \mathcal{Y}} \Lambda(h_i(Y), h_i(I_\text{q})).
\end{equation}
If a patch in the query image contains scene change it will have small histogram intersections with any of the synthetic views, leading to smaller 2D scores.
Note that for computing Equation~\ref{eq:2d} we use the fast histogram generation from Section~\ref{sec:fast} to compute $h_i(Y)$ and avoid the direct rendering of $Y$. 

We utilize the 2D score map to attenuate image regions with changes during candidate pose selection. 
Let $\mathcal{Y}_\text{c}$ denote the $N_f \times N_r$ synthetic views used for finding candidate poses.
We weight the patch-wise histogram intersection using the 2D score map.
For a synthetic view $Y \in \mathcal{Y}_c$, the weighted histogram intersection $w(Y)$ with the query image $I_\text{q}$ is expressed as follows,
\begin{equation}
\label{eq:intersect}
    w(Y) = \sum_i M_i \Lambda(h_i(Y), h_i(I_\text{q})).
\end{equation}
Note that the $\text{i}^\text{th}$ patch-wise histogram intersection is weighted with the corresponding score $M_i$ from the 2D score map.
Since the scores for patches in $I_\text{q}$ that contain change will be low, we can expect these regions to be attenuated in the candidate pose selection process.
We rank the candidate poses based on the intersection values and select the top $K$ poses for further refinement.

\paragraph{3D Score Map}
The 3D score map $M_\text{3D} \in \mathbb{R}^{N}$ measures the color consistency of each  3D point with respect to the query image.
We compute the 3D score map by back-projecting color histogram intersections to the point cloud, as shown in Figure~\ref{fig:score3d}.
Given a synthetic view $Y \in \mathcal{Y}$, let $B_Y \in \mathbb{R}^{N}$ denote the back-projected histogram intersections between patches in $Y$ and $I_\text{q}$.
The 3D score map is the intersections averaged across synthetic views, namely
\begin{equation}
\label{eq:3d}
    M_\text{3D} = \frac{1}{|\mathcal{Y}|} \sum_{Y \in \mathcal{Y}} B_Y.
\end{equation}
If a region in the point cloud contains scene changes, one can expect majority of the back-projected histogram intersections $B_Y$ for that region to be small, leading to smaller 3D scores.
We use the 3D score map for weighting the sampling loss in Equation~\ref{eq:samp_loss}.
By placing smaller weights on regions that contain scene changes, the 3D score map leads to more stable convergence in the pose refinement procedure.
We verify the efficacy of the 2D, 3D score maps for CPO in Section~\ref{exp:abl}.

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}

   \caption{Description of 3D score map generation.}
   \label{fig:score3d}
\end{figure}

\if 0
The 3D score map $M_\text{3D} \in \mathbb{R}^{N}$ similarly measures the color consistency of each  point in the point cloud $X$ with respect to the query image.
For point $\mathbf{x_i} \in X$, we define the 3D score $M_\text{3D, i}$ as the average histogram intersection between the query image and the synthetic view patches containing projections of $\mathbf{x_i}$.
% $b(i; Y)$ is the index of the patch in synthetic view $Y$ where the 2D projection of $\mathbf{x_i}$ resides.
Given a synthetic view $Y \in \mathcal{Y}$, let $b(i; Y)$ be the index of the patch containing the 2D projected $\mathbf{x_i}$.
The 3D score is expressed as follows,
\begin{equation}
    M_\text{3D, i} = \frac{1}{|\mathcal{Y}|}
    \sum_{Y \in \mathcal{Y}}\Lambda(h_{b(i; Y)}(Y), h_{b(i; Y)}(I)).
\end{equation}
\fi


==> table/ablation_sequential_hist.tex <==
% use graph rather than table

\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        {} & \multicolumn{2}{c|}{$t$-error (m)} & \multicolumn{2}{c|}{$R$-error($^\circ$)} & \multicolumn{2}{c}{Acc.}\\
        Method & Robot & Hand & Robot & Hand & Robot & Hand \\
        \midrule
        PICCOLO & 2.948 & 3.370 & 85.0 & 96.5 & 0.18 & 0.08\\
        PICCOLO \footnotesize{w/ prior} & 0.017 & 0.012 & 0.27 & 0.23 & 0.69 & 0.81\\
        CPO \footnotesize{w/o filtering} & 0.005 & 0.008 & 0.10 & 0.12 & 0.89 & 0.79\\
        CPO & 0.006 & 0.008 & 0.12 & 0.13 & 0.89 & 0.80\\
        CPO \footnotesize{w/ prior} & 0.006 & 0.007 & 0.11 & 0.12 & 0.92 & 0.88\\
        \bottomrule
    \end{tabular}
    }
    \caption{ablation study on sequential hist}
    \label{table:ablation_sequential_hist}
\end{table}


==> table/result_matterport.tex <==
\if 0
\begin{table}[t]
    \centering
    % \newcolumntype{C}{>{\centering\arraybackslash}X}
    % \renewcommand*{\arraystretch}{0.95}
    %\setlength{\tabcolsep}{2pt}
    {\small
    \begin{tabularx}{0.85\columnwidth}{l|ccc}
        \toprule
        Method & $t$-error (m) & $R$-error ($^{\circ}$) & Acc.\\
        \midrule
        PICCOLO~\cite{piccolo} & 1.00 & 22.73 & 0.44\\
        CPO & \textbf{0.75} & \textbf{15.44} & \textbf{0.47} \\
        \bottomrule
    \end{tabularx}
    }
    
    \caption{Localization performance of CPO and PICCOLO evaluated on MatterPort3D dataset~\cite{matterport}.}
    \label{table:matterport}
\end{table}
\fi

\begin{table}[t]
    \centering
    % \newcolumntype{C}{>{\centering\arraybackslash}X}
    % \renewcommand*{\arraystretch}{0.95}
    %\setlength{\tabcolsep}{2pt}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        Method & $t$-error (m) & $R$-error ($^{\circ}$) & Accuracy\\
        \midrule
        PICCOLO~\cite{piccolo} & 1.00 & 22.73 & 0.44\\
        CPO & \textbf{0.75} & \textbf{15.44} & \textbf{0.47} \\
        \bottomrule
    \end{tabular}
    }
    
    \caption{Localization performance of CPO and PICCOLO evaluated on MatterPort3D dataset~\cite{matterport}.}
    \label{table:matterport}
\end{table}

==> table/result_mpo.tex <==

\begin{table}[t]
    \centering
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        {} & \multicolumn{2}{c|}{$t$-error (m)} & \multicolumn{2}{c|}{$R$-error ($^\circ$)} & \multicolumn{2}{c}{Accuracy}\\
        Area & PICCOLO & CPO & PICCOLO & CPO & PICCOLO & CPO \\
        \midrule
        Urban & \textbf{0.03} & \textbf{0.03} & 0.85 & \textbf{0.77} & 0.85 & \textbf{0.86} \\
        Coast & 0.79 & \textbf{0.02} & 2.18 & \textbf{0.99} & 0.40 & \textbf{0.68} \\
        Forest & \textbf{0.02} & \textbf{0.02} & 0.92 & \textbf{0.73} & 0.67 & \textbf{0.91} \\
        Parking In & 2.77 & \textbf{0.01} & 96.50 & \textbf{0.66} & 0.13 & \textbf{0.99} \\
        Parking Out & 1.74 & \textbf{0.02} & 9.77 & \textbf{0.82} & 0.07 & \textbf{0.68}\\
        Residential & 0.83 & \textbf{0.02} & 2.53 & \textbf{0.74} & 0.46 & \textbf{0.89}\\
        \midrule
        All & 0.80 & \textbf{0.02} & 2.10 & \textbf{0.76} & 0.45 & \textbf{0.84}\\
        \bottomrule
    \end{tabular}
    }
    \caption{Localization error and accuracy of CPO and PICCOLO on all areas of the Multi-Modal Panoramic 3D Outdoor (MPO) dataset~\cite{fukuoka}.}
    \label{table:mpo}
\end{table}

==> table/result_stanford_all.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.62\linewidth}{!}{
    \begin{tabular}{l|cc}
        \toprule
        Method & $t$-error (m) & $R$-error ($^\circ$) \\
        \midrule
        PoseNet & 2.41 & 28.0  \\
        SphereNet & 2.29 & 26.7 \\
        Zhang et al. & 1.64 & 9.15 \\
        PICCOLO & 0.03 & 0.66 \\
        \midrule
        CPO & 0.01 & 0.24\\
        \bottomrule
    \end{tabular}
    }
    \caption{stanford comparison}
    \label{table:stanford_comparison}
\end{table}

